Guaranteed Conservation of Momentum for Learning Particle-based Fluid Dynamics

We present a novel method for guaranteeing linear momentum in learned physics simulations. Unlike existing methods, we enforce conservation of momentum with a hard constraint, which we realize via antisymmetrical continuous convolutional layers. We combine these strict constraints with a hierarchical network architecture, a carefully constructed resampling scheme, and a training approach for temporal coherence. In combination, the proposed method allows us to increase the physical accuracy of the learned simulator substantially. In addition, the induced physical bias leads to significantly better generalization performance and makes our method more reliable in unseen test cases. We evaluate our method on a range of different, challenging fluid scenarios. Among others, we demonstrate that our approach generalizes to new scenarios with up to one million particles. Our results show that the proposed algorithm can learn complex dynamics while outperforming existing approaches in generalization and training performance. An implementation of our approach is available at https://github.com/tum-pbs/DMCF.

==> Guaranteed Conservation of Momentum for Learning Particle-based Fluid Dynamics-4/introduction.tex <==
\section{Introduction}


Learning physics simulations with machine learning techniques opens up 
a wide range of intriguing paths 
to predict the dynamics of complex physical phenomena such as fluids \cite{morton2018deep,liLearningParticleDynamics2019,ummenhofer2019lagrangian,sanchez2020learning}. As traditional simulators for fluids employ handcrafted simplifications \cite{pope2000turbulent} and require vast amounts of computational resources \cite{tezduyar1996flow}, recent learning-based methods have shown highly promising results. In face of the impressive performance and accuracy of these techniques, it is surprising to see that they still neglect some of the most basic physical principles, like the symmetries that arise from Newton's third law of motion and the conservation of momentum.
This makes learned simulators less predictable and can lead to severe implications when basing decisions on the simulation outcomes.

Predicting physical properties with neural networks is commonly treated as a regression problem \cite{mohan2019compressed,wang2020towards,wiewel2020latent}, where the training signal is defined as a soft constraint.
This simple and desirable formulation allows to effectively learn and approximate physical processes but also gives way to unwanted shortcuts that deviate from the basic laws of physics.
At the same time network architectures are usually designed with generalizability in mind, 
e.g., with applications ranging from geometry processing \cite{qi2017pointnet++} to physical simulations \cite{battaglia2016interaction}.
In contrast, we propose a lean and efficient architecture that provides a stable and large receptive field, while adhering to the desired physical constraints. At training time, we dynamically take the unrolled evolution of the physical state into account to ensure stability when training with longer sequences.

For the implementation of the inductive bias, our approach is inspired by \emph{Smoothed Particle Hydrodynamics} (SPH) methods \cite{gingold1977smoothed,KBST19}, where physical properties are preserved by the appropriate design of the smoothing kernels \cite{BONET199997}.
Our method uses learned convolution kernels that have inherent benefits over general graph structures in the context of physics simulations, as they can easily process positional information.
Instead of using a soft constraint, e.g., by integration into the loss function, our method enforces physical properties by using inductive biases while keeping the simple training signal of a regression problem.
To this end, we integrate symmetries, which are an integral part of the underlying physical models, into our neural network.
This results in guaranteed conservation of momentum for our method.



==> Guaranteed Conservation of Momentum for Learning Particle-based Fluid Dynamics-4/related_work.tex <==
\subsection{Related Work}


Numerical computation of fluid-based dynamics is a long and extensively treated topic in research \cite{harlow1955machine,wilcox1998turbulence}.
We discuss the most relevant work here, and refer to surveys \cite{koschier2022survey} for a full review.
Our approach uses a Lagrangian viewpoint, where fluids are represented as smoothed particles.
This viewpoint by design conserves the mass of the fluid, as the number of particles does not change, and limits valuable computation time to where the fluid is.
This idea stems from astrophysics
\cite{gingold1977smoothed} and is known as \emph{Smoothed Particle Hydrodynamics} (SPH).
It was followed by a large number of papers that improved the SPH method in terms of accuracy and performance \cite{Becker2007,solenthaler2009predictive,macklin2013position,bender2016divergence,hu2019difftaichi,adami2012}.

In contrast to many classic simulators that use sophisticated and handcrafted \nt{model equations} to describe the motion of fluids, our method belongs to the class of data-driven solvers, which entirely learns their dynamics from observations.
A seminal example of learning fluid simulation from data is Ladicky et al. \cite{ladicky2015data}, which uses carefully designed density features with random forests to regress fluid motions. However, the method does not guarantee momentum conservation.
In recent work, algorithms have been proposed to use physical priors based on Lagrangians \cite{saemundsson2020,  lutter2019, cramer2020} or Hamiltonians \cite{sanchez2019hamiltonian} to improve the physical accuracy of learning ODEs and PDEs, and compliance with conservation laws. Nevertheless, the methods are limited to low-dimensional problems and do not address complex PDEs such as those required for fluids.
Other works have used convolutional neural networks, or ConvNets, to achieve acceleration for grid-based fluid simulations  \cite{tompson2016accelerating,um2020solver,kochkov2021machine}.
The former proposes ConvNets to accelerate the expensive pressure correction step \cite{tompson2016accelerating},
while the other two propose ConvNets learning corrections to reduce the grid size and, consequently, the runtime of simulations.
Although these methods show large speed-ups, they inherently cannot be applied to particle-based simulations.

For processing point clouds, the community has followed multiple strategies to address the challenges with this representation.
A key challenge is the permutation invariance of particles. 
An approach to address this uses a combination of point-wise MLPs, order-independent set functions, and farthest point sampling to create a point cloud hierarchy \cite{qi2017pointnet++}.  
Another line of work processes point clouds with graph neural networks.
These methods represent fluid particles with graph nodes and define edges between them \cite{battaglia2016interaction,liLearningParticleDynamics2019,sanchez2020learning}.
Here, interaction networks with relation-centric and object-centric functions were developed to predict future object states \cite{battaglia2016interaction}.
Since the framework aims to be general and employs unconstrained MLPs, it cannot be guaranteed that interactions are symmetric.
The same holds for Li et al. \cite{liLearningParticleDynamics2019}, which uses the same framework and builds a dynamic graph connecting nearby particles to model fluids.
SPH simulations can also be treated as 
\nt{message-passing on graphs \cite{sanchez2020learning, pfaff2020learning, brandstetter2022message}.} 
These approaches typically decompose a simulator into multiple MLPs, which act as encoder, processor, and decoder.
The processor performs multiple rounds of general message-passing, updates node and edge features, and does not enforce physical properties like momentum conservation.
Further, graph-based methods are strongly tied to the chosen particle discretization, and changes to it, like the sampling density, may require non-trivial changes to the models.

As an alternative to explicit graph representations, convolutional architectures represent an interesting option for particle-based simulation.
Schenck et al.~\cite{schenckSPNetsDifferentiableFluid2018} implement special layers for particle-particle interactions and particle-boundary interactions.
The work does not aim to learn a general fluid simulator but implements a differentiable position-based fluids (PBF) \cite{macklin2013position} solver, which is used to estimate liquid parameters or train networks to solve control problems by backpropagation through the solver. Moreover, Fourier neural operators \cite{li2020fourier} or their adaptive variants \cite{guibas2021afno} have been proposed to solve PDEs.
Most related to our approach is Ummenhofer et al.~\cite{ummenhofer2019lagrangian}, which implements a trainable continuous convolution operator resulting in compact networks.
The learned kernels describe general continuous functions with a smooth radial falloff but do not account for symmetric interactions of particles.
We extend the continuous convolutions to enable simulations that guarantee momentum conservation and introduce a particle hierarchy for better accuracy and robustness.

Symmetries play an essential role in physics, as isolated systems are invariant to certain transformations, i.e., the behavior of a physical system does not depend on its orientation. For example, Lie point symmetries were used to optimize data augmentation and thus improve the sample efficiency for learning PDEs \cite{brandstetter2022pointsym}.
Similar observations apply for the structural analysis of molecules \cite{eismann2021hierarchical} and vision applications \cite{symconv,Son_2020_ACCV}.
The chemical properties of proteins do not change under rotation, nor should class labels of objects in images.
Rotationally equivariant architectures have been proposed to leverage this concept for improved generalization and sample efficiency, e.g., constraining the convolution kernels for the $E(2)$ group to achieve equivariance \cite{weiler2019general}. A similar approach by Wang et al.~\cite{wang2020incorporating} was applied to physics-based problems.
Kernel constraints can also be transferred to continuous convolutions on 2D point clouds for improved sample efficiency of traffic trajectory predictions \cite{walters2020trajectory}.
For 3D problems, spherical harmonics can be used to define rotationally equivariant filters \cite{thomas2018tensor}, which shows their application to shape classification, molecule generation, and simple problems in classical mechanics.
The method guarantees rotational equivariance, but filter evaluations can become expensive for higher degrees.
In addition, architectures for symmetries in arbitrary dimensions were proposed \cite{villar2021scalars,satorras2021n}, which however require graph-based representations.






